Accountable and Explainable Methods for Complex Reasoning over Text

A major concern of Machine Learning (ML) models is their opacity. They are deployed in an increasing number of applications where they often operate as black boxes that do not provide explanations for their predictions. Among others, the potential harms associated with the lack of understanding of the models' rationales include privacy violations, adversarial manipulations, and unfair discrimination. As a result, the accountability and transparency of ML models have been posed as critical desiderata by works in policy and law, philosophy, and computer science. In computer science, the decision-making process of ML models has been studied by developing accountability and transparency methods. Accountability methods, such as adversarial attacks and diagnostic datasets, expose vulnerabilities of ML models that could lead to malicious manipulations or systematic faults in their predictions. Transparency methods explain the rationales behind models' predictions gaining the trust of relevant stakeholders and potentially uncovering mistakes and unfairness in models' decisions. To this end, transparency methods have to meet accountability requirements as well, e.g., being robust and faithful to the underlying rationales of a model. This thesis presents my research that expands our collective knowledge in the areas of accountability and transparency of ML models developed for complex reasoning tasks over text.

==> frontbackmatter/bibliography.tex <==
\chapter{Bibliography}
\vspace{1cm}
\printbibliography[heading=none]

==> frontbackmatter/quotes.tex <==
% \vspace*{4cm}
% \textit{"I want to say a word for the study of comparative physiology also for its own sake. You will find in the lower animals mechanisms and adaptations of exquisite beauty and the most surprising character, and I think nothing can be more fascinating than the senses and instincts of insects as revealed by the modern investigations."} \\
% \newline
% \rightline{August Krogh, 1929 \nocite{Krogh1929}} \\
% \vspace{2cm}
% \newline
% \textit{"It is certain that there may be extraordinary mental activity with an extremely small absolute mass of nervous matter: thus the wonderfully diversified instincts, mental powers, and affections of ants are notorious, yet their cerebral ganglia are not so large as the quarter of a small pin's head. Under this point of view, the brain of an ant is one of the most marvelous atoms of matter in the world, perhaps more so than the brain of a man."} \\
% \newline
% \rightline{Charles Darwin, 1872 \nocite{Darwin1872TheSex}}
% \vspace{3.8cm}




==> frontbackmatter/titlepage.tex <==
% Cover back page
\AddToShipoutPicture*{\TitleWatermark}% adding watermark
\hfill
\vfill
{
	\small
	\textbf{\thesisName} \\
	\textit{\thesisTitle} \\
	\thesisSubject, \thesisDate \\
	Supervisors: \thesisExternalSupervisor\ and \thesisInternalSupervisor \\[1.5em]
	\textbf{\thesisUniversity} \\
	\textit{\thesisFaculty} \\
	\thesisInstitute \\
	\thesisAddress \\
	\thesisPostal\ \thesisCity
}


==> mainmatter/8_diagnostic_study_nles.tex <==
\chapter{diagnostic study nles}
\label{chap:diagnostic_study_nles}


==> mainmatter/9_interactive_explanations.tex <==
\chapter{interactive explanations}
\label{chap:interactive_explanations}

